Deep Reinforcement Learning Attitude Control of Fixed-Wing UAVs Using Proximal Policy Optimization

Contemporary autopilot systems for unmanned aerial vehicles (UAVs) are far more limited in their flight envelope as compared to experienced human pilots, thereby restricting the conditions UAVs can operate in and the types of missions they can accomplish autonomously. This paper proposes a deep reinforcement learning (DRL) controller to handle the nonlinear attitude control problem, enabling extended flight envelopes for fixed-wing UAVs. A proof-of-concept controller using the proximal policy optimization (PPO) algorithm is developed, and is shown to be capable of stabilizing a fixed-wing UAV from a large set of initial conditions to reference roll, pitch and airspeed values. The training process is outlined and key factors for its progression rate are considered, with the most important factor found to be limiting the number of variables in the observation vector, and including values for several previous time steps for these variables. The trained reinforcement learning (RL) controller is compared to a proportional-integral-derivative (PID) controller, and is found to converge in more cases than the PID controller, with comparable performance. Furthermore, the RL controller is shown to generalize well to unseen disturbances in the form of wind and turbulence, even in severe disturbance conditions.

==> sections/abstract_old.tex <==
Contemporary autopilot systems for \glspl{uav} are far more limited in their flight envelope as compared to experienced human pilots, thereby restricting the conditions \glspl{uav} can operate in and the types of missions they can accomplish autonomously. Autopilot systems typically consists of an inner loop attitude controller providing stabilization, and one or more outer control loops governing mission objectives. The inner loop has traditionally been based on the \gls{pid} controller, due to its transparency and near optimal performance in normal flight conditions. However, since the \gls{pid} controller assumes the underlying dynamics are described in linear terms, it is only able to provide stabilization for some subset of flight conditions, and this is a considerable source of the discrepancy between autopilot and human pilot. This paper proposes a \gls{rl} controller as a candidate to handle the nonlinear attitude control problem and extended flight envelopes for fixed-wing \glspl{uav}. A proof-of-concept controller using the \gls{drl} algorithm \gls{ppo} is developed, and is shown to be capable of stabilizing a fixed-wing aircraft from a large set of initial conditions to a desired attitude reference. The training process is outlined and key factors for its progression rate are considered, with the most important factor found to be limiting the size of the state vector to the essential information. The trained \gls{rl} controller is shown to generalize well to unseen and unmodeled disturbances in the form of wind and turbulence, even with severe disturbance magnitudes.

==> sections/approach_old.tex <==
\section{APPROACH/METHOD} \label{sec:approach}
\gls{ppo} was chosen as the \gls{rl} algorithm for the attitude controller for a couple of reasons: first, \gls{ppo} was found to be the best performing algorithm for attitude control of quadcopters in \cite{koch_reinforcement_2018}, and secondly, \gls{ppo} is the default choice of algorithm in OpenAI applications, because of its high performance and low computational intensity. 

The objective is to control the \glspl{uav} attitude, so a natural choice of controlled variables are the roll, pitch and yaw angles. However, the Skywalker X8 is an underactuated system, and the yaw of the aircraft is therefore typically not controlled directly. In addition, it is desirable to stay close to some nominal airspeed due to efficiency reasons, to avoid stall, and to maintain control surface effectiveness which is proportional to airspeed squared. The \gls{rl} controller is therefore tasked with controlling the roll and pitch angles, $\phi$ and $\theta$, as well as the airspeed $V_a$ to desired setpoints. The controller has at its disposal the control surfaces of the aircraft, here the elevons of the Skywalker X8, and the propeller throttle. The action space of the controller is therefore three dimensional, consisting of the elevator and aileron angles, both between $-30\degree$ and $35\degree$, and the throttle setpoint between 0 and 1. 

While the environment has access to perfect estimates of all states in the simulation, feeding all this information to the controller would not be a realistic representation of real world flight, and might not even be productive. The choice of what components go into the observation vector is therefore based on what is reasonably attainable in the field, as well as the information's impact on controller performance.

\subsection{Training of Controller}

\begin{table}
    \caption{Constraints and ranges for initial conditions and target setpoints used during training of controller.}
    \centering
    \ra{1.2}
    \begin{tabular}{@{}lrrr@{}} \toprule
    Variable & Initial Condition & Target & Constraint \\  \midrule
    $\phi$ & $\pm 60\degree$ & $\pm 30\degree$ & - \\
    $\theta$ & $\pm 30\degree$ & $\pm 20\degree$ & $\pm 85\degree$ \\
    $\psi$ & $\pm 60\degree$ & - & - \\
    $\omega_{1, 2, 3}$ & $\pm 0.7 rad/s$ & - & $\pi rad/s$ \\
    $V^b$ & [$10-25$, $\pm 5$, $\pm 5$]$m/s$ & - & - \\
    $V_a$ & $12-30 m/s$ & $12-30 m/s$ & - \\
    %Wind & $[\pm 8, \pm 8, \pm 8] m/s$ & - & - \\
    $\beta$ & - & - & $\pm 85\degree$ \\ 
    \bottomrule
    \end{tabular}
    \label{tab:training_variables}
\end{table}

The \gls{ppo} \gls{rl} controller was initialized with the default hyperparameters in the OpenAI baselines implementation \cite{stable-baselines}. Different values of the nsteps parameter were explored, as is discussed in the results and discussion section, but also here the default value seemed to give the best performance. The controller policy is also the default option: a simple \gls{nn} comprised of two fully connected layers of 64 neurons each, with hyperbolic tangent activation functions. The initial state of the \gls{uav} was randomized in a moderate range around stable flight conditions for each episode, and the same is true for the references. Through considering the typical report rate of the sensors aboard a \gls{uav}, found to be around $100$ hertz, the simulator was chosen to advance $0.01$ seconds at each time step. In order to encourage desirable behaviour of the \gls{uav} and for stability of the simulator, some states were constrained. In particular, to avoid the singularity found in Euler angles, the pitch angle $\theta$ was constrained to $\pm 85 \degree$, moreover the sideslip angle $\beta$ was constrained to $\pm 85 \degree$ and the angular rates $\omega_{\{1, 2, 3\}}$ were constrained to $\pm \pi rad/s$. The initial conditions, targets and constraints are summarized in table \ref{tab:training_variables}. Each episode is terminated after a maximum of 500 time steps, corresponding to 5 seconds of real world flight time, or when one of the state constraints are violated.

\begin{align}\label{eq:rew}
    r_{attitude} &= clip(\frac{|\phi - \phi_{target}| + |(\theta - \theta_{target})|}{\zeta_1}, 0, \gamma_1) \nonumber \\
    r_{V_a} &= clip(\frac{|V_a - V_{a_{target}}|}{\zeta_2}, 0, \gamma_2) \nonumber \\
    r_\omega &= clip(\frac{\sum_{i=1}^3 |\omega_i|}{\zeta_3}, 0, \gamma_3) \nonumber \\
    r_t &= -(r_{attitude} + r_{V_a} + r_\omega)
\end{align}
\begin{align}
    \zeta_1 &= 2.5,~\zeta_2 = 30,~~ \zeta_3 = 3 \nonumber \\
    \gamma_1 &= 0.6,~ \gamma_2 = 0.3,~ \gamma_3 = 0.1 \nonumber
\end{align}


In accordance with traditional control literature where one usually considers cost to be minimized rather than rewards to be maximized, the reward returns to the \gls{rl} controller are all negative rewards in the normalized range of -1 to 0. In the reward function shown in \eqref{eq:rew} the $L_1$ norm was chosen as the distance metric between current state and desired state, and is also used to punish high angular rates. The importance of each components are weighted through the gamma factors. To balance the disparate scales of the velocity target and the attitude targets, the setpoint error is divided by the variables approximate dynamic range, represented by the zeta factors. Another important aspect of the reward structure to consider is how to handle premature termination of the episode due to constraint violations. With no additional punishment for these situations, an alluring solution for the \gls{rl} controller would be to steer the aircraft towards one of the constraints in as few time steps as possible, as this would give a low total punishment. To discourage these types of strategies the \gls{rl} controller receives an additional punishment equal to the amount of steps left in the simulation when the episode is terminated due to constraint violation. This solution breaks the paradigm of normalized rewards in the range of -1 to 0, but seems to work well as the policy will receive very steep negative gradients for actions which lead to these constraint-violating trajectories. 

The components of the state vector are expressed in different units and also have differing dynamic ranges. \glspl{nn} are known to converge faster when the input features share a common scale, such that the network does not need to learn this scaling itself. The observation vector should therefore be normalized. This is accomplished with the VecNormalize class of \cite{stable-baselines}, which estimates the mean and variance of each component as the agent learns and normalizes based on these estimates.

\subsection{Evaluation}
To evaluate the \gls{rl} controllers performance in a consistent manner across a wide array of initial conditions, targets and wind conditions, 100 episodes with a set initial condition, target and wind are generated and used to evaluate the controller. Each test episode consists of a step response of magnitude 10 to 20 degrees for the angle variables, and 1 to 5 m/s for the airspeed. For the test cases with atmospheric disturbances, wind and turbulence forces are randomized for each episode with a set magnitude, up to severe conditions according to \cite{dryden}, i.e. around 23 m/s at a height of 20 foot. Each episode is run for a maximum of 250 time steps, corresponding to $2.5$ seconds of flight time, which should be sufficient time to allow the controller to achieve the setpoint and also showcase its stability capabilities in terms of settling at the setpoint.

As is discussed in the preceding section, the reward function is not merely measuring the proficiency of the \gls{rl} controller, but is also designed to facilitate learning. To compare, rank and evaluate different version of the \gls{rl} controller, one needs to define additional evaluation criteria. To this end, the controllers are evaluated on the following criteria: \textbf{Success/failure} whether the controller is successful in controlling the attitude to within some bound of the setpoint, the attitude must stay within the bounds for at least the last 10 \% of the time steps to be counted as a success. The bound was chosen to be $\pm 5\degree$ for the roll and pitch angles, and $\pm 2 m/s$ for the airspeed. \textbf{Rise time}, the time it takes the controller to reduce the initial error from 90 \% to 10 \%. As these control scenarios are not just simple step responses and may cross these thresholds several times during the episode, the rise time is calculated from the first time it crosses the lower threshold until the first time it reaches the upper threshold. \textbf{Settle time}, the time it takes the controller to settle within the setpoint bounds, and never leave this bound again. \textbf{Overshoot}, the peak value reached on the opposing side of the setpoint wrt. the initial error, expressed as a percentage of the initial error. Rise time, settle time and overshoot are only measured when the episode is counted as a success.

Comparing the \gls{rl} controller with a \gls{pid} controller would be informative and help highlight the good and bad characteristics of the \gls{rl} controller. However, the necessary time to properly tune a \gls{pid} controller to ensure a fair comparison could not be set aside.

==> sections/conclusion.tex <==
\section{CONCLUSIONS} \label{sec:conclusion}
The ease with which the proof of concept \gls{rl} controller learns to control the \gls{uav} for the tasks presented in this paper, and its ability to generalize to turbulent wind conditions, suggests that \gls{drl} is a good candidate for nonlinear flight control design. A central unanswered question here is the severity of the reality gap, or in other words how transferable the strategies learned in simulations are to real world flight. Future work should evaluate the controller's robustness to parametric and structural aerodynamic uncertainties; this is essential to do before undertaking any real life flight experiments. For more advanced maneuvers, e.g. aerobatic flight or recovering from extreme situations, the controller should be given more freedom in adjusting the airspeed, possibly through having it as an uncontrolled state. 

There is still much potential left to harness for this class of controllers. The policy network used to represent the control law is small and simple; more complex architectures such as \gls{lstm} could be used to make a dynamic \gls{rl} controller. Training, experiments and reward structures can be designed to facilitate learning of more advanced behavior, tighter control or better robustness. Should the reality gap prove to be a major obstacle for the success of the \gls{rl} controller in the real world, one should look to the class of off-policy algorithms such as \gls{sac}. These algorithms are able to learn offline from gathered data, and thus might be more suited for \gls{uav} applications. 
%%
%Due to the risks involved in data collection with \gls{uav} systems, one should consider off-policy algorithms such as \gls{sac}, which is able to learn offline from gathered data.

%Other \gls{drl} algorithms could have properties that are desirable in this context, e.g. the off-policy \gls{sac} algorithm which is able to learn offline from gathered data, which might be more suited for an aircraft application.

% TODO: maybe talk about SAC and better suited through offline learning

%\myworries{Nevne også reward function expereimentering i future work...}

% \myworries{Noe om tracking?} 

%\myworries{Nevne det at man bør prøve å la airspeed være ukontrollert, dvs la attitude control få full kontroll over throttle også for ekstreme attitude maneuvers. Også evaluere controller for extreme maneuvers er future work}\myworries{Litt mye ny info i konklusjonen?} 

==> sections/introduction_old.tex <==
\section{INTRODUCTION}\label{sec:introduction} 

\begin{figure}[thpb]
        \includegraphics[width=0.48\textwidth]{figs/FlyingX8.pdf}
        \caption{Skywalker X8 Fixed Wing UAV}
        \label{fig:x8}
\end{figure}

\glspl{uav} are employed extensively to increase safety and efficiency in a plethora of tasks such as building and industrial inspection, forest monitoring and search and rescue missions. Many tasks can however not be accomplished fully autonomously, due to several limitations of autopilot systems. Low-level stabilization of the \gls{uav}s attitude provided by the inner control loop is increasingly difficult as the attitude deviates from stable level conditions. The outer control loop providing path planning and navigation has to bear this in mind, and settle for conservative and safe plans. Equipping the autopilot with the low-level stabilization skills of an experienced pilot would allow fully autonomous operation in dangerous or otherwise troublesome environments, such as search and rescue missions in extreme weather conditions, as well as increasing the usefulness of the drone by for instance allowing the drone to fly closer to its targets for inspection purposes.

%The workhorse behind the inner loop of conventional autopilots, the ubiquitous \gls{pid} controller, is linear in its nature and therefore requires the highly non-linear aerodynamics affecting the aircraft during flight to be linearized. This idealization introduces artifacts which are major contributing factors in the described discrepancy between a human pilot and the autopilot. The accuracy of the linearized model quickly degrades when diverging from the linearization point, necessitating several linearized models and accompanying \gls{pid} controller gains for different operating circumstances, with subsequent switching effects.
Autopilots for fixed-wing \glspl{uav} are typically designed using cascaded single-variable loops under assumptions of decoupled longitudinal and lateral motion, using classical linear control theory~\cite{Beard}. The dynamics of fixed-wing aircraft including \glspl{uav} are however strongly coupled and nonlinear. Nonlinear terms in the equations of motion include kinematic nonlinearities (rotations and coriolis effects), actuator saturation and aerodynamic nonlinearities, which are also highly uncertain and difficult to model. The decoupled and linear designs are reliable and well-tested for nominal flight, but also requires conservative safety limits in the allowable range of flight conditions and maneuvers (flight envelope protection), because linear controllers applied to nonlinear systems typically result in a limited region of attraction~\cite{Khalil2001}. This motivates the use of state-of-the-art nonlinear control algorithms.

Examples of nonlinear control methods applied to \glspl{uav} include gain scheduling~\cite{Girish2014}, linear parameter varying (LPV) control~\cite{Rotondo2017}, dynamic inversion (feedback linearization)~\cite{Kawakami2017}, adaptive backstepping~\cite{Sonneveldt2007}~\cite{Ren2005}, sliding mode control~\cite{Castaneda2017}, nonlinear model predictive control~\cite{Mathisen2016}, nonlinear H-infinity control~\cite{Garcia2017}, mu-synthesis~\cite{Michailidis2017} and model reference adaptive control~\cite{EugeneLavretsky2012}. Several of these methods require a more or less accurate aerodynamic model of the UAV. A model-free method based on fuzzy logic can be found in~\cite{Kurnaz2008}. Fuzzy control falls under the category of intelligent control systems, which also includes the use of neural networks. An adaptive backstepping controller using a neural network to compensate for aerodynamic uncertainties is given in~\cite{Lee2001}, while a genetic neuro-fuzzy approach for attitude control is taken in~\cite{Oliveira2017}. The state of the art in intelligent flight control of small \glspl{uav} is discussed in~\cite{Santoso2018}.

%\gls{ml} methods therefore seem like a natural candidate to be involved in some capacity of the improved autopilot, whether it be in a system identification role or directly in the control aspect.
\gls{ml} methods have shown great promise in uncovering intricate models from data and representing complex nonlinear relations from its inputs to its outputs. \gls{ml} methods that learn from scratch can be made free from designer bias and dubious assumptions about the underlying process, while simultaneously being adaptable to new systems and environments through retraining. \gls{drl}, an emerging field combining the power of \glspl{nn} with \gls{rl} frameworks, has recently been applied with great success to classical control problems such as the inverted pendulum problem, as well as more complex tasks such as motion control of robots~\cite{Zhang} and video game playing \cite{mnih_human-level_2015}. While simpler approaches such as the prominent \gls{pid} controller is inherently reactive, such that an error has to occur before it can be remedied, a \gls{ml} based controller can act as a predictive system, a feature predominantly shared by approaches more computationally and knowledge intense such as the \gls{mpc}.

The premise of this research project was to explore the application of \gls{rl} methods to low-level control of fixed-wing drones, in the hopes of producing a proof-of-concept \gls{rl} controller capable of stabilizing the attitude of the \acrshort{uav} to a given reference vector. To this end, an OpenAI  gym~\cite{brockman_openai_2016} environment with a high-fidelity aerodynamics simulator tailored to the x8 Skywalker was implemented. The gym environment with the goal of deriving a \gls{rl} controller capable of controlling the attitude (here, the roll, pitch and air velocity) of the aircraft. The aerodynamics simulator was designed with the goal of being valid for a wide array of flight conditions, and therefore includes nonlinear extensions of standard models corresponding with experimental wind tunnel data from \cite{Gryte}. Key factors impacting the final performance of the controller as well as the rate of progression during training were identified. To the best of the authors' knowledge, this is the first work to use \gls{rl} for attitude control of fixed-wing \glspl{uav}.

The rest of the paper is organized as follows. First, theoretical background of the \gls{rl} methods and frameworks are presented in section \ref{sec:background}, and previous applications of \gls{rl} algorithms to \glspl{uav} are presented in section \ref{sec:related}. The aerodynamic model of the Skywalker X8 fixed wing aircraft is then introduced in section \ref{sec:model}. Section \ref{sec:approach} outlines the approach taken to develop the \gls{rl} controller, presenting the configurations of the \gls{rl} algorithm and the key design decisions taken, and finally describing how the controller is evaluated. In section \ref{sec:results}, the training process and its major moments are presented and discussed, and the controller is evaluated in light of the approach described in the preceding section. Finally, section \ref{sec:conclusion} offers some closing thoughts on the papers subject and suggests further work to be done.

%\myworries{Point out that the method is model-free and training is done using simulation and not real life flight.}

==> sections/model_old_equations.tex <==
\section{UAV MODEL} \label{sec:model}
The UAV is modeled as a rigid body of mass $m$ with inertia tensor $\boldsymbol{I}_g$ and a body frame $\{b\}$ rigidly attached to its center of mass, moving relative to a north-east-down (NED) frame assumed to be inertial $\{n\}$. The time evolution of the position $\boldsymbol{p}^n_{b/n}= \begin{bmatrix} x & y & z \end{bmatrix}^T$ and attitude $\boldsymbol{\Theta}_{nb}$ of the UAV is governed by the kinematic equations
\begin{align}
\dot{\boldsymbol{p}}^n_{b/n}   &= \boldsymbol{R}^n_b (\boldsymbol{\Theta}_{nb}) \boldsymbol{v}^b_{b/n} \\
\dot{\boldsymbol{\Theta}}_{nb}   &= \boldsymbol{T}_\Theta(\boldsymbol{\Theta}_{nb}) \boldsymbol{\omega}^b_{b/n}
\end{align}
The attitude is represented using Euler angles $\boldsymbol{\Theta}_{nb} = [\phi,\theta,\psi]$, where $\phi$, $\theta$, $\psi$ are the roll, pitch and yaw angles respectively. The Euler angle transformation matrix $\boldsymbol{T}_{\boldsymbol{\Theta}} (\boldsymbol{\Theta}_{nb} )$ relating the angular velocity $\boldsymbol{\omega}^b_{b/n} = \begin{bmatrix} p & q & r\end{bmatrix}^T$ to the time derivative of the Euler angles can be calculated from $\boldsymbol{\Theta}_{nb}$ as follows:
\begin{equation}
\boldsymbol{T}_{\boldsymbol{\Theta}}(\boldsymbol{\Theta}_{nb}) = 
\begin{bmatrix}
1 & \sin\phi \tan \theta & \cos \phi \tan \theta \\
0 & \cos \phi & -\sin \phi \\
0 & \sin \phi \sec \theta & \cos \phi \sec \theta
\end{bmatrix}
\end{equation}
The rotation matrix $\boldsymbol{R}^n_b$ transforms vectors from $\{b\}$ to $\{n\}$ and is given by the following sequence of basic rotations:
\begin{equation}
\boldsymbol{R}^n_b(\boldsymbol{\Theta}) = \boldsymbol{R}_{z,\psi} \boldsymbol{R}_{y,\theta} \boldsymbol{R}_{x,\phi}
\end{equation}
The rates of change of the body-fixed velocities $\boldsymbol{v}^b_{b/n}$ and angular velocities are given by the Newton-Euler equations of motion:
\begin{align}
m ( \dot{\boldsymbol{v}}^b_{b/n} + \boldsymbol{\omega}^b_{b/n} \times \boldsymbol{v}^b_{b/n} )&= m (\boldsymbol{R}^n_b) ^T\boldsymbol{g}^n + \boldsymbol{F}_{prop}^b+\boldsymbol{F}_{aero}^b\\
\boldsymbol{I}_g\dot{\boldsymbol{\omega}}^b_{b/n} + \boldsymbol{\omega}^b_{b/n} \times (\boldsymbol{I}_g \boldsymbol{\omega}^b_{b/n})&=  \boldsymbol{M}^b_{prop} + \boldsymbol{M}^b_{aero}
\end{align}
$\boldsymbol{g}^n = \begin{bmatrix} 0 & 0 & g\end{bmatrix}^T$, where $g$ is the acceleration of gravity. Apart from gravity, the UAV is affected forces and moments due to propulsion and aerodynamics, that are explained in the next sections.

\subsection{Aerodynamic Forces and Moments}
The UAV is flying in a wind field decomposed into a steady part $\boldsymbol{v}_{w_s}^n$ and a stochastic part $\boldsymbol{v}^b_{w_g}$ representing gusts and turbulence. The relative (to the surrounding airmass) velocity of the UAV is then defined as
\begin{equation}
\boldsymbol{v}_r^b = \boldsymbol{v}_{b/n}^b - (\boldsymbol{R}^n_b)^T\boldsymbol{v}^n_{w_s} - \boldsymbol{v}^n_{w_g} = \begin{bmatrix}
u_r \\ v_r \\ w_r
\end{bmatrix}
\end{equation}
From the relative velocity we can calculate the airspeed $V_a$, angle of attack $\alpha$ and sideslip angle $\beta$:
\begin{align}
V_a &= \sqrt{u_r^2 + v_r^2 + w_r^2 } \\
\alpha &= \tan^{-1}\left(\frac{u_r}{w_r}\right)  \\
\beta &= \sin^{-1}\left(\frac{v_r}{V_a}\right)
\end{align}

The stochastic part of the wind, including rotational components, is generated by passing white noise through shaping filters given by the Dryden velocity spectra~\cite{dryden}.

%\begin{align}
%    H_u(s)  &= \sigma_u  \sqrt{\frac{2 L_u}{\pi V_a}} \frac{1}{1 + \frac{L_u}{V_a}s} \\
%    H_v(s)  &= \sigma_v  \sqrt{\frac{L_v}   {\pi V_a}} \frac{1 + \frac{\sqrt{3}L_v}{V_a}s}{\left(1 + \frac{L_v}{V_a}s\right)^2} \\
%    H_w(s) &= \sigma_w \sqrt{\frac{L_w}  {\pi V_a}} \frac{1+ \frac{\sqrt{3}L_w}{V_a}s}{\left(1 + \frac{L_w}{V_a}s\right)^2} 
%\end{align}
%\begin{align}
%    H_p (s) &= \sigma_w \sqrt{\frac{0.8}{V_a}}\frac{\frac{\pi}{4b}^{\frac{1}{6}}}{L_w^{\frac{1}{3}}\left( 1 + \frac{4b}{\pi V_a}s\right)} \\
%    H_q (s) &= - \frac{\frac{s}{V_a}}{1 + \frac{4b}{\pi V_a}s} \cdot H_w(s) \\
%    H_r (s)  &=   \frac{\frac{s}{V_a}}{1 + \frac{3b}{\pi V_a}s} \cdot H_v(s) \\ 
%\end{align}
%The parameters of the spectra are the turbulence intensities $\sigma_{(*)}$ and length scales $L_{*}$ given by
%\begin{align}
%\sigma_w &= 0.1 W_{20} \\
%\sigma_u &= \sigma_v = \frac{\sigma_w}{\left( 0.177 + 0.000823h \right)^{0.4}} \\
%L_u  &= L_v = \frac{h}{\left(  0.177 + 0.000823h\right)^{1.2}} \\
%L_w &= h
%\end{align}
%$W_{20}$ is the wind speed at 20 feet  and $h = -z$ is the altitude.

The aerodynamic forces and moments are formulated in terms of aerodynamic coefficients $C_{(*)}$ that are, in general, nonlinear functions of $\alpha$, $\beta$ and $\boldsymbol{\omega}_{b/n}^b$, as well as the right and left elevon surface deflections $\delta_{e,r}$ and $\delta_{e,l}$, which acts as control inputs. Note that there is no rudder on the Skywalker X8 \gls{uav} that is considered here.

\begin{figure}[thpb]
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[scale=0.3]{figs/dryden/dryden_lin.pdf}
        \caption{Linear velocity}
        \label{fig:dryden:lin}
    \end{subfigure}
    ~\begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[scale=0.3]{figs/dryden/dryden_ang.pdf}
        \caption{Angular velocity}
        \label{fig:dryden:ang}
    \end{subfigure}
    \caption{Realizations of the Dryden turbulence model for severe turbulence conditions.}
    \label{fig:dryden}
\end{figure}

\begin{align}
\boldsymbol{F}_{aero}^b &= \boldsymbol{R}^b_w(\alpha,\beta)\begin{bmatrix} 
-D \\Y \\ -L
\end{bmatrix} \\
\begin{bmatrix} 
D  \\ Y \\ L
\end{bmatrix} &= \frac{1}{2}\rho V_a^2S  \begin{bmatrix} C_D(\alpha,\beta,q,\delta_{e,r},\delta_{e,l}) \\ C_Y(\beta,p,r,\delta_{e,r},\delta_{e,l}) \\ C_L(\alpha,q,\delta_{e,r},\delta_{e,l})\end{bmatrix} \\
\boldsymbol{M}^b_{aero}  &= \frac{1}{2}\rho V_a^2S\begin{bmatrix}
bC_l(\beta,p,r,\delta_{e,r},\delta_{e,l}) \\ cC_m(\alpha,q,\delta_{e,r},\delta_{e,l}) \\ bC_n(\beta,p,r,\delta_{e,r},\delta_{e,l})
\end{bmatrix}
\end{align}
$\rho$ is the density of air, $S$ is the wing planform area, $c$ is the aerodynamic chord, and $b$ the wingspan of the UAV.
The rotation matrix transforming the drag force $D$, side force $Y$ and lift force $L$ from the wind frame to the body frame is given by:
\begin{equation}
\boldsymbol{R}^b_w(\alpha,\beta) = \begin{bmatrix}
\cos(\alpha)\cos(\beta) & \cos(\alpha)\sin(\beta) & -\sin(\alpha) \\-\sin(\beta) & \cos(\beta) & 0 \\
\cos(\beta)\sin(\alpha) & \sin(\alpha)\sin(\beta) & \cos(\alpha)
\end{bmatrix}
\end{equation}
Aerodynamic coefficients are taken from~\cite{Gryte}, based on wind tunnel experiments of the Skywalker X8 flying wing. The model has similar structure to the linear coefficients in~\cite{Beard}, but has added quadratic terms in $\alpha$ and $\beta$ to the drag coefficient $C_D$. In addition, $C_D$ is quadratic in the elevator deflection $\delta_e$. As an attempt to extend the range of validity to a greater range of $\alpha$ and $\beta$-values, lift, drag and pitch moment coefficients are made nonlinear using Newtonian flat plate theory from \cite{Beard} and \cite{Gryte2015}.

\subsection{Propulsion Forces and Moments}
Assuming the propeller thrust is aligned with the x-axis of $\{b\}$, we can write
\begin{equation}
\boldsymbol{F}^b_{prop} = \begin{bmatrix} T_p \\ 0 \\ 0\end{bmatrix}
\end{equation}
Where the propeller thrust $T_p$ is given by~\cite{Beard}:
\begin{align}
V_d   &= V_a + \delta_t (k_m - V_a) \\
T_p   &= \frac{1}{2}\rho S_p C_p V_d \left(V_d - V_a \right)
\end{align}
$V_d$ is the discharge velocity of air from the propeller, $k_m$ is a motor constant, $S_p$ is the propeller disc area, and $C_p$ is an efficiency factor. $\delta_t \in [0,1]$ is the throttle.
The propeller moments are given by
\begin{equation}
\boldsymbol{M}^b_{prop} = \begin{bmatrix} -k_Q (k_\Omega \delta_t)^2 \\ 0 \\ 0\end{bmatrix}
\end{equation}
where $k_\Omega$ and $k_Q$ are constants. Gyroscopic moments are assumed negligible.

\subsection{Actuator Dynamics and Constraints}
Note that  collective and differential elevon deflections can be mapped to "virtual" aileron and elevator deflections $\delta_a$ and $\delta_e$ which are used as input to the aerodynamic model.
\begin{equation}
\begin{bmatrix}
\delta_a \\ \delta_e
\end{bmatrix} = \begin{bmatrix}
-0.5 & 0.5 \\ 0.5 & 0.5
\end{bmatrix} \begin{bmatrix}
\delta_{e,r} \\ \delta_{e,l}
\end{bmatrix}
\end{equation}

For simplicity, constraints and dynamics are imposed on the transformed aileron and elevator deflections. $\delta_a \in [-30\frac{\pi}{180},30\frac{\pi}{180}]$ and $\delta_e \in [-30\frac{\pi}{180},35\frac{\pi}{180}]$.

Denoting commands with superscript c, the control surface dynamics are given by the following second order transfer function:
\begin{equation}
    \frac{\delta_{(*)}(s)}{\delta^c_{(*)}(s)} = \frac{\omega_0^2}{s^2 + 2\zeta \omega_0 s + \omega_0^2}
\end{equation}
where $\omega_0$ is the natural frequency, and $\zeta$ a damping factor. The throttle dynamics are given by the following first order transfer function:
\begin{equation}
    \frac{\delta_t(s)}{\delta_t^c(s)} = \frac{1}{T_{\delta_t} s + 1}
\end{equation}
where $T_{\delta_t}$ is some time constant.

==> sections/related_old.tex <==
\section{RELATED WORK} \label{sec:related}
%Fixed-wing aircraft are normally underactuated vehicles, i.e. not actuated in all directions in 3D space. Guidance of such vehicles along a desired path is typically performed by controlling the attitude (orientation) and speed. For most aircraft, the magnitude of the lift force is typically larger than the thrust force (\myworries{kilde}). Heading changes are therefore most efficiently done by banking and thus tilting the lift force out of the vertical plane, creating a centripetal force for turning (bank-to-turn). Similarily, altitude changes can be made by controlling the flight path angle through the pitch angle. The inner-loop consists of linear \gls{pid} controllers for roll and pitch angles. The primary controls for roll are the aileron control surfaces, while an elevator provides pitching moments. Some \glspl{uav} also have a tail with a rudder that can produce yawing moments, which are typically used to minimize sideslip when turning (coordinated turn).
There has generally been little application of \gls{rl} to \gls{uav} platforms compared to other robotics applications due to the high sample complexity of \gls{rl} frameworks, and the difficulty of acquiring real world data due to crashes often being fatal. \gls{rl} has been proposed as solutions to many high level tasks for \acrshortpl{uav} such as the higher level path planning and navigation tasks, while tried and tested traditional controllers are used in conjunction for low-level stabilization. The work of~\citet{gandhiLearning2017} goes counter to the notion stated earlier, as they teach a \gls{uav} to navigate in an indoor environment by gathering a sizable dataset consisting of crashes, giving the \gls{uav} ample experience of how NOT to fly. In~\cite{Han}, the authors tackle the data collection problem by constructing a pseudo flight environment in which the \gls{uav} and the surrounding area is fitted with magnets, allowing for adjustable magnetic forces and moments in each \gls{dof}. In this way, the \gls{uav} can be propped up as one would do when teaching a baby to walk, and thereby experiment without fear of crashing in a setting more realistic than simulations.

\citet{Imanberdiyev2016} developed a model-based \gls{rl} algorithm called TEXPLORE to efficiently plan trajectories in unknown environments subject to constraints such as battery life.~\citet{Pham2018} uses a model-free Q-learning approach in combination with \gls{pid} controllers for attitude control of the quadcopter to navigate an unknown environment to a target point.~\citet{Kelchtermans2017} trained a \gls{rnn} to directly map from sensory camera data to navigation instructions, in order to avoid obstacles in the \glspl{uav} planned path. In~\cite{ZhangMPC}, the authors use an \gls{mpc} to generate training data for a \gls{rl} controller, thereby guiding the policy search and avoiding the potentially catastrophic phase before an effective policy is found. Their controller generalizes to avoid multiple obstacles, compared to the singular obstacle avoided by the \gls{mpc} in training, does not require full state information like the \gls{mpc} does, and is computed at a fraction of the time. ~\citet{Hwangbo2017} uses a \gls{drl} algorithm for waypoint tracking of quadrotors, coupled with \gls{pid} controllers for attitude stabilization. They found that the computation time of \gls{nn} controllers were two orders of magnitude lower than the traditional alternatives.
% Hwangbo They also developed a new learning algorithm which is deterministic on-policy method (not very revolutionary now)

With the advent of \gls{drl}, it has also been used for more advanced tasked such as enabling intelligent cooperation between multiple \glspl{uav}~\cite{Hung2017}, and for specific control tasks such as landing:~\citet{Polvara2018} proposes to employ a hierarchy of \glspl{dqn} to map from camera data to control input for landing \glspl{uav} autonomously in a wide range of conditions. \gls{rl} algorithms have also been proposed for attitude control of other autonomous vehicles, including satellites~\cite{Xu2018} and underwater vehicles.~\citet{Carlucho2018} applies an actor-critic \gls{drl} algorithm to low-level attitude control of an \gls{auv}, similar to the proposed method in this paper. They also obtain experimental data from testing their method on the Nessie VII \gls{auv} and find satisfactory result in terms of the transferability from simulation training to the real world performance.

Of work addressing problems more similar in nature to the one in this paper, i.e. low-level attitude control, one can trace the application of \gls{rl} methods back to the 2001 and 2004 works of~\citet{Bagnell} and~\citet{Ng}, both focusing on traditional helicopter \glspl{uav}. Both employed methods based on learning offline from data gathered by an experienced pilot. The former focuses on control of a subset of the controllable states while keeping the others fixed, whereas the latter work extends the control to all six degrees of freedom. Both experiment with the methods in practice and find that the algorithms are capable of control performance exceeding that of the original pilot. In~\cite{Abbeel}, the latter work was further extended to include difficult acrobatic maneuvers such as forward flips and sideways rolls, significantly improving upon the state of the art.  In 2010,~\citet{Bou-Ammar2010} compared a \gls{rl} algorithm using \gls{fvi} to a non-linear controller based on feedback linearization on their proficiency in stabilizing a quadcopter \gls{uav} after an input disturbance, finding the non-linear controller to have the superior performance. Recently,~\citet{koch_reinforcement_2018} applied the \gls{ppo} algorithm along with others to attitude control of the angular rates of a quadcopter \gls{uav}. They found \gls{ppo} to perform the best of the \gls{rl} algorithms, even outperforming the \gls{pid} controller on nearly every metric. 
